HypothesisMed: Inference-Time Answer Fusion and Structured Hypothesis-Space Reporting for Biomedical Question Answering

Biomedical question answering with large language models is commonly evaluated using answer accuracy, but answer accuracy alone does not indicate whether a model can produce parseable outputs, follow structured reliability instructions, recognize weak answer spaces, or avoid confident incorrect commitments. This paper presents HypothesisMed, an inference-time reliability pipeline for biomedical multiple-choice question answering. It combines direct, chain-of-thought, HypothesisMed-v3 prompting, and answer fusion. The final answer is selected by fusion, while HypothesisMed-v3 supplies SPACE labels and confidence information. SPACE labels mark the answer space as VALID, INCOMPLETE, or CONTRADICTED. We evaluate Qwen2.5-7B, Phi-4-mini, DeepSeek-R1-32B, and BioMistral-7B on MedQA, MedMCQA, and PubMedQA using 1,000 examples per dataset. The pipeline improves weighted accuracy over each model's best direct or chain-of-thought baseline while increasing parse and SPACE coverage. We also scale evaluation to Qwen2.5-7B and Phi-4-mini using 10,183 examples per model. Fusion improves Phi-4-mini accuracy from 0.4296 to 0.5192, while Qwen2.5-7B chain-of-thought remains slightly higher in answer accuracy. However, Qwen2.5-7B fusion achieves complete parse and SPACE coverage with much lower false commitment. A 12,000-example SPACE stress test shows answer-space diagnosis remains difficult, with SPACE accuracy of 0.3074 for Qwen2.5-7B and 0.4168 for Phi-4-mini. These results show that answer accuracy, parseability, structured reliability reporting, calibration behavior, and false-commitment behavior are separable capabilities. The main contribution is not a universal state-of-the-art claim, but a reproducible inference-time framework for evaluating biomedical question answering models as auditable workflow components under structured reliability constraints.

==> paper_assests/tables/confidence_accuracy_by_dataset.tex <==
% Auto-generated from CSV. Do not edit manually unless needed.
\begin{tabular}{llll}
\toprule
dataset & mean\_confidence & accuracy & n \\
\midrule
medmcqa & 0.1208 & 0.3885 & 4000 \\
medqa & 0.1282 & 0.3845 & 4000 \\
pubmedqa & 0.2201 & 0.5258 & 4000 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/confidence_rows_from_fusion_outputs_first30.tex <==
% Auto-generated from CSV. Do not edit manually unless needed.
\begin{tabular}{lllll}
\toprule
file & model & dataset & confidence & correct \\
\midrule
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 1 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 1 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 1 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 1 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 0 \\
results/fusion/biomistral\_biomistral\_7b\_fusion\_majority\_answer\_hypmed\_v3\_space\_medmcqa\_original1000.jsonl & biomistral\_biomistral\_7b & medmcqa & 0 & 1 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/ready_table_blocks_for_paper.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage{longtable}

\begin{table*}[t]
\centering
\caption{Aggregate four-model results across MedQA, MedMCQA, and PubMedQA. Higher answer accuracy, parse coverage, and SPACE coverage are better. Lower false commitment is better.}
\label{tab:aggregate}
\resizebox{\textwidth}{!}{%
\input{paper_assests/tables/table_main_4model_aggregate_clean.tex}
}
\end{table*}

\begin{table*}[t]
\centering
\caption{Accuracy and reliability deltas of the proposed method compared with each model's best direct or chain-of-thought baseline.}
\label{tab:deltas}
\resizebox{\textwidth}{!}{%
\input{paper_assests/tables/table_deltas_vs_baseline_clean.tex}
}
\end{table*}

\begin{table*}[t]
\centering
\caption{Per-dataset results for the proposed answer-fusion plus HypothesisMed-v3 SPACE method. Each row uses 1,000 examples.}
\label{tab:perdataset}
\resizebox{\textwidth}{!}{%
\input{paper_assests/tables/table_proposed_per_dataset_clean.tex}
}
\end{table*}

\begin{table}[t]
\centering
\caption{Confidence and accuracy summary by dataset for the proposed fusion outputs.}
\label{tab:confidence_dataset}
\resizebox{\linewidth}{!}{%
\input{paper_assests/tables/confidence_accuracy_by_dataset.tex}
}
\end{table}

% Optional appendix table. Use only if you want example-level confidence rows.
% For this one, add \usepackage{longtable}.
\begin{table*}[t]
\centering
\caption{Example-level confidence rows from proposed fusion outputs, truncated to the first 30 rows for readability.}
\label{tab:confidence_rows}
\resizebox{\textwidth}{!}{%
\input{paper_assests/tables/confidence_rows_from_fusion_outputs_first30.tex}
}
\end{table*}


==> paper_assests/tables/table_deltas_vs_baseline_clean.tex <==
% Auto-generated from CSV. Do not edit manually unless needed.
\begin{tabular}{llllllllllllll}
\toprule
model & proposed\_accuracy & baseline\_name & baseline\_accuracy & absolute\_accuracy\_gain & relative\_accuracy\_gain\_percent & proposed\_parse\_coverage & baseline\_parse\_coverage & proposed\_space\_coverage & baseline\_space\_coverage & proposed\_false\_commitment & baseline\_false\_commitment & false\_commitment\_reduction & model\_clean \\
\midrule
Qwen2.5-7B-Instruct & 0.6367 & Chain-of-thought & 0.6003 & 0.0364 & 6.06 & 1 & 0.944 & 0.9997 & 0.002 & 0.1026 & 0.8478 & 0.7452 & Qwen2.5-7B \\
Phi-4-mini-instruct & 0.5767 & Chain-of-thought & 0.4817 & 0.095 & 19.72 & 0.9913 & 0.7923 & 0.992 & 0 & 0.4054 & 0.9838 & 0.5784 & Phi-4-mini \\
DeepSeek-R1-Distill-Qwen-32B & 0.3877 & Direct & 0.169 & 0.2187 & 129.41 & 0.7213 & 0.3557 & 0.443 & 0.001 & 0.0213 & 0.2986 & 0.2773 & DeepSeek-R1-32B \\
biomistral\_biomistral\_7b & 0.1307 & Chain-of-thought & 0.1247 & 0.006 & 4.81 & 0.333 & 0.3203 & 0.004 & 0 & 0 & 0.8287 & 0.8287 & BioMistral-7B \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_expanded_space_stress_by_gold_label.tex <==
\begin{tabular}{llrrr}
\toprule
Model & Gold SPACE & N & Coverage & Accuracy \\
\midrule
Qwen2.5-7B & CONTRADICTED & 6000 & 1.000000 & 0.257300 \\
Qwen2.5-7B & INCOMPLETE & 3000 & 1.000000 & 0.091000 \\
Qwen2.5-7B & VALID & 3000 & 1.000000 & 0.624000 \\
Phi-4-mini & CONTRADICTED & 6000 & 0.983700 & 0.348200 \\
Phi-4-mini & INCOMPLETE & 3000 & 0.994300 & 0.450000 \\
Phi-4-mini & VALID & 3000 & 0.992300 & 0.520700 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_expanded_space_stress_by_stress_type.tex <==
\begin{tabular}{llrrr}
\toprule
Model & Stress type & N & Coverage & Accuracy \\
\midrule
Qwen2.5-7B & CONTRADICTED\_AMBIGUOUS\_NONUNIQUE\_OPTION & 3000 & 1.000000 & 0.132000 \\
Qwen2.5-7B & CONTRADICTED\_DUPLICATE\_CORRECT\_OPTION & 3000 & 1.000000 & 0.382700 \\
Qwen2.5-7B & INCOMPLETE\_REMOVE\_CORRECT & 3000 & 1.000000 & 0.091000 \\
Qwen2.5-7B & VALID\_ORIGINAL & 3000 & 1.000000 & 0.624000 \\
Phi-4-mini & CONTRADICTED\_AMBIGUOUS\_NONUNIQUE\_OPTION & 3000 & 0.988300 & 0.356000 \\
Phi-4-mini & CONTRADICTED\_DUPLICATE\_CORRECT\_OPTION & 3000 & 0.979000 & 0.340300 \\
Phi-4-mini & INCOMPLETE\_REMOVE\_CORRECT & 3000 & 0.994300 & 0.450000 \\
Phi-4-mini & VALID\_ORIGINAL & 3000 & 0.992300 & 0.520700 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_expanded_space_stress_confusion_counts.tex <==
\begin{tabular}{lllr}
\toprule
Model & Gold SPACE & Pred SPACE & Count \\
\midrule
Qwen2.5-7B & CONTRADICTED & CONTRADICTED & 1544 \\
Qwen2.5-7B & CONTRADICTED & INCOMPLETE & 75 \\
Qwen2.5-7B & CONTRADICTED & VALID & 4381 \\
Qwen2.5-7B & INCOMPLETE & CONTRADICTED & 1787 \\
Qwen2.5-7B & INCOMPLETE & INCOMPLETE & 273 \\
Qwen2.5-7B & INCOMPLETE & VALID & 940 \\
Qwen2.5-7B & VALID & CONTRADICTED & 1055 \\
Qwen2.5-7B & VALID & INCOMPLETE & 73 \\
Qwen2.5-7B & VALID & VALID & 1872 \\
Phi-4-mini & CONTRADICTED & CONTRADICTED & 2089 \\
Phi-4-mini & CONTRADICTED & INCOMPLETE & 3369 \\
Phi-4-mini & CONTRADICTED & NONE & 98 \\
Phi-4-mini & CONTRADICTED & VALID & 444 \\
Phi-4-mini & INCOMPLETE & CONTRADICTED & 62 \\
Phi-4-mini & INCOMPLETE & INCOMPLETE & 1350 \\
Phi-4-mini & INCOMPLETE & NONE & 17 \\
Phi-4-mini & INCOMPLETE & VALID & 1571 \\
Phi-4-mini & VALID & CONTRADICTED & 17 \\
Phi-4-mini & VALID & INCOMPLETE & 1398 \\
Phi-4-mini & VALID & NONE & 23 \\
Phi-4-mini & VALID & VALID & 1562 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_expanded_space_stress_overall.tex <==
\begin{tabular}{lrrr}
\toprule
Model & N & SPACE coverage & SPACE accuracy \\
\midrule
Qwen2.5-7B & 12000 & 1.000000 & 0.307400 \\
Phi-4-mini & 12000 & 0.988500 & 0.416800 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_main_4model_aggregate_clean.tex <==
% Auto-generated from CSV. Do not edit manually unless needed.
\begin{tabular}{llllllllll}
\toprule
Model & Method & Datasets & N & answer\_accuracy & parse\_coverage & space\_coverage & false\_commitment & model\_clean & method\_clean \\
\midrule
Qwen2.5-7B-Instruct & Proposed: answer fusion + HypothesisMed-v3 SPACE & 3 & 3000 & 0.6367 & 1 & 0.9997 & 0.1026 & Qwen2.5-7B & Proposed \\
Qwen2.5-7B-Instruct & Chain-of-thought & 3 & 3000 & 0.6003 & 0.944 & 0.002 & 0.8478 & Qwen2.5-7B & CoT \\
Qwen2.5-7B-Instruct & Direct & 3 & 3000 & 0.565 & 0.9147 & 0.0007 & 0.9255 & Qwen2.5-7B & Direct \\
Qwen2.5-7B-Instruct & HypothesisMed-v3 & 3 & 3000 & 0.5623 & 0.986 & 0.9997 & 0.0973 & Qwen2.5-7B & HypMed-v3 \\
Phi-4-mini-instruct & Proposed: answer fusion + HypothesisMed-v3 SPACE & 3 & 3000 & 0.5767 & 0.9913 & 0.992 & 0.4054 & Phi-4-mini & Proposed \\
Phi-4-mini-instruct & Chain-of-thought & 3 & 3000 & 0.4817 & 0.7923 & 0 & 0.9838 & Phi-4-mini & CoT \\
Phi-4-mini-instruct & Direct & 3 & 3000 & 0.302 & 0.5403 & 0 & 0.8329 & Phi-4-mini & Direct \\
Phi-4-mini-instruct & HypothesisMed-v3 & 3 & 3000 & 0.4943 & 0.931 & 0.992 & 0.4341 & Phi-4-mini & HypMed-v3 \\
DeepSeek-R1-Distill-Qwen-32B & Proposed: answer fusion + HypothesisMed-v3 SPACE & 3 & 3000 & 0.3877 & 0.7213 & 0.443 & 0.0213 & DeepSeek-R1-32B & Proposed \\
DeepSeek-R1-Distill-Qwen-32B & Chain-of-thought & 3 & 3000 & 0.071 & 0.237 & 0.001 & 0 & DeepSeek-R1-32B & CoT \\
DeepSeek-R1-Distill-Qwen-32B & Direct & 3 & 3000 & 0.169 & 0.3557 & 0.001 & 0.2986 & DeepSeek-R1-32B & Direct \\
DeepSeek-R1-Distill-Qwen-32B & HypothesisMed-v3 & 3 & 3000 & 0.3413 & 0.5793 & 0.443 & 0.0266 & DeepSeek-R1-32B & HypMed-v3 \\
biomistral\_biomistral\_7b & Proposed: answer fusion + HypothesisMed-v3 SPACE & 3 & 3000 & 0.1307 & 0.333 & 0.004 & 0 & BioMistral-7B & Proposed \\
biomistral\_biomistral\_7b & Chain-of-thought & 3 & 3000 & 0.1247 & 0.3203 & 0 & 0.8287 & BioMistral-7B & CoT \\
biomistral\_biomistral\_7b & Direct & 3 & 3000 & 0.008 & 0.0147 & 0 & 0.131 & BioMistral-7B & Direct \\
biomistral\_biomistral\_7b & HypothesisMed-v3 & 3 & 3000 & 0.0007 & 0.004 & 0.004 & 0 & BioMistral-7B & HypMed-v3 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_proposed_per_dataset_clean.tex <==
% Auto-generated from CSV. Do not edit manually unless needed.
\begin{tabular}{llllllllll}
\toprule
dataset & model & n & answer\_accuracy & ci95 & parse\_coverage & space\_coverage & space\_accuracy & false\_commitment & model\_clean \\
\midrule
medmcqa & Qwen2.5-7B-Instruct & 1000 & 0.561 & [0.530, 0.592] & 1 & 1 & 0.635 & 0.0501 & Qwen2.5-7B \\
medmcqa & Phi-4-mini-instruct & 1000 & 0.489 & [0.458, 0.520] & 0.997 & 0.994 & 0.5191 & 0.3465 & Phi-4-mini \\
medmcqa & DeepSeek-R1-Distill-Qwen-32B & 1000 & 0.34 & [0.311, 0.369] & 0.819 & 0.26 & 0.9923 & 0.0522 & DeepSeek-R1-32B \\
medmcqa & biomistral\_biomistral\_7b & 1000 & 0.164 & [0.141, 0.187] & 0.476 & 0.011 & 0 & 0 & BioMistral-7B \\
medqa & Qwen2.5-7B-Instruct & 1000 & 0.596 & [0.566, 0.626] & 1 & 0.999 & 0.4324 & 0.1361 & Qwen2.5-7B \\
medqa & Phi-4-mini-instruct & 1000 & 0.517 & [0.486, 0.548] & 0.99 & 0.982 & 0.4216 & 0.2156 & Phi-4-mini \\
medqa & DeepSeek-R1-Distill-Qwen-32B & 1000 & 0.255 & [0.228, 0.282] & 0.594 & 0.404 & 0.995 & 0.0118 & DeepSeek-R1-32B \\
medqa & biomistral\_biomistral\_7b & 1000 & 0.17 & [0.147, 0.193] & 0.42 & 0.001 & 1 & 0 & BioMistral-7B \\
pubmedqa & Qwen2.5-7B-Instruct & 1000 & 0.753 & [0.726, 0.780] & 1 & 1 & 0.906 & 0.1215 & Qwen2.5-7B \\
pubmedqa & Phi-4-mini-instruct & 1000 & 0.724 & [0.696, 0.752] & 0.987 & 1 & 0.92 & 0.654 & Phi-4-mini \\
pubmedqa & DeepSeek-R1-Distill-Qwen-32B & 1000 & 0.568 & [0.537, 0.599] & 0.751 & 0.665 & 0.997 & 0 & DeepSeek-R1-32B \\
pubmedqa & biomistral\_biomistral\_7b & 1000 & 0.058 & [0.044, 0.072] & 0.103 & 0 &  & 0 & BioMistral-7B \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_scaled_compact_comparison.tex <==
\begin{tabular}{p{1.5cm}p{1.3cm}p{1.25cm}p{1.4cm}p{1.5cm}p{1.4cm}p{1.4cm}p{1.4cm}}
\toprule
Model & Best baseline & Baseline acc. & Fusion acc. & $\Delta$ acc. & Parse cov. & SPACE cov. & False commit. \\
\midrule
Phi-4-mini & CoT & 0.4296 & 0.5192 & 0.0896 & 0.9928 & 0.9905 & 0.3271 \\
Qwen2.5-7B & CoT & 0.6079 & 0.5953 & -0.0126 & 1.0000 & 1.0000 & 0.1146 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_scaled_fallback_order_sensitivity.tex <==
\begin{tabular}{lllrrr}
\toprule
Model & Dataset & Fallback order & N & Parse coverage & Accuracy \\
\midrule
Qwen2.5-7B & MedQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 5000 & 1.000000 & 0.593000 \\
Qwen2.5-7B & MedQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 5000 & 1.000000 & 0.589400 \\
Qwen2.5-7B & MedQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 5000 & 1.000000 & 0.602400 \\
Qwen2.5-7B & MedQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 5000 & 1.000000 & 0.601400 \\
Qwen2.5-7B & MedQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 5000 & 1.000000 & 0.582000 \\
Qwen2.5-7B & MedQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 5000 & 1.000000 & 0.582000 \\
Qwen2.5-7B & MedMCQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 4183 & 1.000000 & 0.560400 \\
Qwen2.5-7B & MedMCQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 4183 & 1.000000 & 0.558000 \\
Qwen2.5-7B & MedMCQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 4183 & 1.000000 & 0.566300 \\
Qwen2.5-7B & MedMCQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 4183 & 1.000000 & 0.566300 \\
Qwen2.5-7B & MedMCQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 4183 & 1.000000 & 0.553400 \\
Qwen2.5-7B & MedMCQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 4183 & 1.000000 & 0.555100 \\
Qwen2.5-7B & PubMedQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 1000 & 1.000000 & 0.753000 \\
Qwen2.5-7B & PubMedQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 1000 & 1.000000 & 0.753000 \\
Qwen2.5-7B & PubMedQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 1000 & 1.000000 & 0.755000 \\
Qwen2.5-7B & PubMedQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 1000 & 1.000000 & 0.755000 \\
Qwen2.5-7B & PubMedQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 1000 & 1.000000 & 0.757000 \\
Qwen2.5-7B & PubMedQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 1000 & 1.000000 & 0.757000 \\
Phi-4-mini & MedQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 5000 & 0.987400 & 0.510400 \\
Phi-4-mini & MedQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 5000 & 0.987400 & 0.477200 \\
Phi-4-mini & MedQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 5000 & 0.987400 & 0.504400 \\
Phi-4-mini & MedQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 5000 & 0.987400 & 0.496200 \\
Phi-4-mini & MedQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 5000 & 0.987400 & 0.460600 \\
Phi-4-mini & MedQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 5000 & 0.987400 & 0.458600 \\
Phi-4-mini & MedMCQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 4183 & 0.997800 & 0.484300 \\
Phi-4-mini & MedMCQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 4183 & 0.997800 & 0.467400 \\
Phi-4-mini & MedMCQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 4183 & 0.997800 & 0.487000 \\
Phi-4-mini & MedMCQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 4183 & 0.997800 & 0.475700 \\
Phi-4-mini & MedMCQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 4183 & 0.997800 & 0.457100 \\
Phi-4-mini & MedMCQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 4183 & 0.997800 & 0.458000 \\
Phi-4-mini & PubMedQA & direct $\rightarrow$ cot $\rightarrow$ hyp & 1000 & 0.999000 & 0.709000 \\
Phi-4-mini & PubMedQA & direct $\rightarrow$ hyp $\rightarrow$ cot & 1000 & 0.999000 & 0.645000 \\
Phi-4-mini & PubMedQA & cot $\rightarrow$ direct $\rightarrow$ hyp & 1000 & 0.999000 & 0.722000 \\
Phi-4-mini & PubMedQA & cot $\rightarrow$ hyp $\rightarrow$ direct & 1000 & 0.999000 & 0.725000 \\
Phi-4-mini & PubMedQA & hyp $\rightarrow$ direct $\rightarrow$ cot & 1000 & 0.999000 & 0.648000 \\
Phi-4-mini & PubMedQA & hyp $\rightarrow$ cot $\rightarrow$ direct & 1000 & 0.999000 & 0.657000 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_scaled_fusion_calibration_bins.tex <==
\begin{tabular}{lllrrrr}
\toprule
Model & Dataset & Bin & N & Mean confidence & Accuracy & Abs gap \\
\midrule
Qwen2.5-7B & MedQA & 0.0-0.1 & 4205 & 0.000000 & 0.578400 & 0.578400 \\
Qwen2.5-7B & MedQA & 0.7-0.8 & 2 & 0.800000 & 0.500000 & 0.300000 \\
Qwen2.5-7B & MedQA & 0.8-0.9 & 30 & 0.893300 & 0.733300 & 0.160000 \\
Qwen2.5-7B & MedQA & 0.9-1.0 & 763 & 0.996000 & 0.668400 & 0.327600 \\
Qwen2.5-7B & MedMCQA & 0.0-0.1 & 3860 & 0.000000 & 0.549500 & 0.549500 \\
Qwen2.5-7B & MedMCQA & 0.4-0.5 & 1 & 0.500000 & 1.000000 & 0.500000 \\
Qwen2.5-7B & MedMCQA & 0.7-0.8 & 2 & 0.775000 & 0.500000 & 0.275000 \\
Qwen2.5-7B & MedMCQA & 0.8-0.9 & 8 & 0.893800 & 0.250000 & 0.643800 \\
Qwen2.5-7B & MedMCQA & 0.9-1.0 & 312 & 0.997800 & 0.701900 & 0.295800 \\
Qwen2.5-7B & PubMedQA & 0.0-0.1 & 759 & 0.000000 & 0.770800 & 0.770800 \\
Qwen2.5-7B & PubMedQA & 0.8-0.9 & 4 & 0.900000 & 0.500000 & 0.400000 \\
Qwen2.5-7B & PubMedQA & 0.9-1.0 & 237 & 0.995800 & 0.700400 & 0.295400 \\
Phi-4-mini & MedQA & 0.0-0.1 & 3084 & 0.000000 & 0.497700 & 0.497700 \\
Phi-4-mini & MedQA & 0.1-0.2 & 1 & 0.200000 & 0.000000 & 0.200000 \\
Phi-4-mini & MedQA & 0.4-0.5 & 327 & 0.500000 & 0.458700 & 0.041300 \\
Phi-4-mini & MedQA & 0.5-0.6 & 23 & 0.600000 & 0.608700 & 0.008700 \\
Phi-4-mini & MedQA & 0.6-0.7 & 19 & 0.649700 & 0.315800 & 0.333900 \\
Phi-4-mini & MedQA & 0.7-0.8 & 52 & 0.761300 & 0.480800 & 0.280600 \\
Phi-4-mini & MedQA & 0.8-0.9 & 486 & 0.896600 & 0.504100 & 0.392500 \\
Phi-4-mini & MedQA & 0.9-1.0 & 945 & 1.000000 & 0.610600 & 0.389400 \\
Phi-4-mini & MedMCQA & 0.0-0.1 & 2584 & 0.000100 & 0.469800 & 0.469700 \\
Phi-4-mini & MedMCQA & 0.4-0.5 & 143 & 0.500000 & 0.531500 & 0.031500 \\
Phi-4-mini & MedMCQA & 0.5-0.6 & 13 & 0.596200 & 0.692300 & 0.096200 \\
Phi-4-mini & MedMCQA & 0.6-0.7 & 6 & 0.650000 & 0.666700 & 0.016700 \\
Phi-4-mini & MedMCQA & 0.7-0.8 & 3 & 0.786700 & 0.333300 & 0.453300 \\
Phi-4-mini & MedMCQA & 0.8-0.9 & 343 & 0.895900 & 0.521900 & 0.374000 \\
Phi-4-mini & MedMCQA & 0.9-1.0 & 1082 & 0.999900 & 0.501800 & 0.498100 \\
Phi-4-mini & PubMedQA & 0.0-0.1 & 889 & 0.000000 & 0.695200 & 0.695200 \\
Phi-4-mini & PubMedQA & 0.4-0.5 & 21 & 0.500000 & 0.666700 & 0.166700 \\
Phi-4-mini & PubMedQA & 0.7-0.8 & 1 & 0.780000 & 1.000000 & 0.220000 \\
Phi-4-mini & PubMedQA & 0.8-0.9 & 7 & 0.850000 & 0.714300 & 0.135700 \\
Phi-4-mini & PubMedQA & 0.9-1.0 & 81 & 1.000000 & 0.876500 & 0.123500 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_scaled_fusion_calibration_summary.tex <==
\begin{tabular}{llrrrrr}
\toprule
Model & Dataset & N & Accuracy & Mean confidence & ECE-10 & Brier \\
\midrule
Qwen2.5-7B & MedQA & 5000 & 0.593000 & 0.157700 & 0.537500 & 0.538200 \\
Qwen2.5-7B & MedMCQA & 4183 & 0.560400 & 0.076600 & 0.530600 & 0.530600 \\
Qwen2.5-7B & PubMedQA & 1000 & 0.753000 & 0.239600 & 0.656600 & 0.657100 \\
Phi-4-mini & MedQA & 4937 & 0.516900 & 0.326100 & 0.431100 & 0.447500 \\
Phi-4-mini & MedMCQA & 4174 & 0.485400 & 0.353400 & 0.452400 & 0.461800 \\
Phi-4-mini & PubMedQA & 999 & 0.709700 & 0.098300 & 0.633300 & 0.635500 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_scaled_mcnemar_exact_tests.tex <==
\begin{tabular}{lllrrrr}
\toprule
Model & Dataset & Baseline & N shared & Fusion correct/base wrong & Base correct/fusion wrong & Exact p \\
\midrule
Qwen2.5-7B & MedQA & CoT & 5000 & 273 & 383 & 0.000020 \\
Qwen2.5-7B & MedMCQA & CoT & 4183 & 265 & 278 & 0.606615 \\
Qwen2.5-7B & PubMedQA & CoT & 1000 & 30 & 35 & 0.620145 \\
Phi-4-mini & MedQA & CoT & 5000 & 578 & 127 & 0.000000 \\
Phi-4-mini & MedMCQA & CoT & 4183 & 607 & 142 & 0.000000 \\
Phi-4-mini & PubMedQA & CoT & 1000 & 27 & 31 & 0.694004 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_scaled_two_model_weighted_aggregate.tex <==
\begin{tabular}{p{2.4cm}p{1.6cm}r p{2.0cm}p{2.0cm}p{2.0cm}p{2.0cm}p{2.0cm}}
\toprule
Model & Method & N & Weighted accuracy & Weighted parse cov. & Weighted SPACE cov. & Weighted SPACE acc. & Weighted false commit. \\
\midrule
Phi-4-mini & CoT & 10183 & 0.4296 & 0.8062 & 0.0000 & 0.0000 & 0.9875 \\
Phi-4-mini & Direct & 10183 & 0.2870 & 0.5567 & 0.0000 & 0.0000 & 0.8652 \\
Phi-4-mini & Fusion & 10183 & 0.5192 & 0.9928 & 0.9905 & 0.4768 & 0.3271 \\
Phi-4-mini & HypMed-v3 & 10183 & 0.3933 & 0.9074 & 0.9905 & 0.4768 & 0.3616 \\
Qwen2.5-7B & CoT & 10183 & 0.6079 & 0.9967 & 0.0000 & 0.0000 & 0.9979 \\
Qwen2.5-7B & Direct & 10183 & 0.5750 & 0.9917 & 0.0000 & 0.0000 & 0.9980 \\
Qwen2.5-7B & Fusion & 10183 & 0.5953 & 1.0000 & 1.0000 & 0.5471 & 0.1146 \\
Qwen2.5-7B & HypMed-v3 & 10183 & 0.4839 & 0.9785 & 1.0000 & 0.5471 & 0.0997 \\
\bottomrule
\end{tabular}

==> paper_assests/tables/table_space_stress_compact.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Model & N & Coverage & Accuracy & VALID rec. & INCOMPLETE rec. & CONTRADICTED rec. \\
\midrule
Qwen2.5-7B & 540 & 0.9963 & 0.5185 & 0.7167 & 0.4111 & 0.4278 \\
Phi-4-mini & 540 & 0.5907 & 0.1833 & 0.4944 & 0.0389 & 0.0167 \\
\bottomrule
\end{tabular}


==> paper_assests/tables/table_structured_output_failure_taxonomy.tex <==
\begin{tabular}{%
>{\centering\arraybackslash}p{1.35cm}
>{\centering\arraybackslash}p{1.45cm}
>{\centering\arraybackslash}p{1.35cm}
>{\centering\arraybackslash}p{0.85cm}
>{\centering\arraybackslash}p{0.75cm}
>{\centering\arraybackslash}p{0.95cm}
>{\centering\arraybackslash}p{0.75cm}
>{\centering\arraybackslash}p{0.95cm}
>{\centering\arraybackslash}p{0.85cm}
>{\centering\arraybackslash}p{0.85cm}
>{\centering\arraybackslash}p{0.75cm}
>{\centering\arraybackslash}p{0.95cm}
>{\centering\arraybackslash}p{0.85cm}}
\toprule
Model & Data & Method & N & AM & AMR & SM & SMR & WPA & CPA & MJ & MJR & HCW \\
\midrule
Qwen2.5 & MedQA & Direct & 5000 & 51 & 0.0102 & 5000 & 1.0000 & 2099 & 2850 & 16 & 0.0032 & 2095 \\
Qwen2.5 & MedQA & CoT & 5000 & 26 & 0.0052 & 5000 & 1.0000 & 1899 & 3075 & 39 & 0.0078 & 1895 \\
Qwen2.5 & MedQA & HypMed & 5000 & 126 & 0.0252 & 0 & 0.0000 & 2576 & 2298 & 4980 & 0.9960 & 285 \\
Qwen2.5 & MedQA & Fusion & 5000 & 0 & 0.0000 & 0 & 0.0000 & 2035 & 2965 & 4980 & 0.9960 & 262 \\
Qwen2.5 & MedMCQA & Direct & 4183 & 34 & 0.0081 & 4183 & 1.0000 & 1891 & 2258 & 11 & 0.0026 & 1886 \\
Qwen2.5 & MedMCQA & CoT & 4183 & 7 & 0.0017 & 4183 & 1.0000 & 1819 & 2357 & 34 & 0.0081 & 1814 \\
Qwen2.5 & MedMCQA & HypMed & 4183 & 93 & 0.0222 & 0 & 0.0000 & 2155 & 1935 & 4179 & 0.9990 & 102 \\
Qwen2.5 & MedMCQA & Fusion & 4183 & 0 & 0.0000 & 0 & 0.0000 & 1839 & 2344 & 4179 & 0.9990 & 100 \\
Qwen2.5 & PubMedQA & Direct & 1000 & 0 & 0.0000 & 1000 & 1.0000 & 253 & 747 & 0 & 0.0000 & 253 \\
Qwen2.5 & PubMedQA & CoT & 1000 & 0 & 0.0000 & 1000 & 1.0000 & 242 & 758 & 0 & 0.0000 & 242 \\
Qwen2.5 & PubMedQA & HypMed & 1000 & 0 & 0.0000 & 0 & 0.0000 & 306 & 694 & 1000 & 1.0000 & 81 \\
Qwen2.5 & PubMedQA & Fusion & 1000 & 0 & 0.0000 & 0 & 0.0000 & 247 & 753 & 1000 & 1.0000 & 73 \\
Phi-4 & MedQA & Direct & 5000 & 2860 & 0.5720 & 5000 & 1.0000 & 1014 & 1126 & 2 & 0.0004 & 785 \\
Phi-4 & MedQA & CoT & 5000 & 944 & 0.1888 & 5000 & 1.0000 & 1955 & 2101 & 0 & 0.0000 & 1939 \\
Phi-4 & MedQA & HypMed & 5000 & 492 & 0.0984 & 77 & 0.0154 & 2541 & 1967 & 4722 & 0.9444 & 1012 \\
Phi-4 & MedQA & Fusion & 5000 & 63 & 0.0126 & 77 & 0.0154 & 2385 & 2552 & 4722 & 0.9444 & 835 \\
Phi-4 & MedMCQA & Direct & 4183 & 1423 & 0.3402 & 4183 & 1.0000 & 1498 & 1262 & 2 & 0.0005 & 1414 \\
Phi-4 & MedMCQA & CoT & 4183 & 1017 & 0.2431 & 4183 & 1.0000 & 1605 & 1561 & 1 & 0.0002 & 1572 \\
Phi-4 & MedMCQA & HypMed & 4183 & 130 & 0.0311 & 20 & 0.0048 & 2285 & 1768 & 3390 & 0.8104 & 886 \\
Phi-4 & MedMCQA & Fusion & 4183 & 9 & 0.0022 & 20 & 0.0048 & 2148 & 2026 & 3390 & 0.8104 & 778 \\
Phi-4 & PubMedQA & Direct & 1000 & 231 & 0.2310 & 1000 & 1.0000 & 234 & 535 & 0 & 0.0000 & 232 \\
Phi-4 & PubMedQA & CoT & 1000 & 13 & 0.0130 & 1000 & 1.0000 & 274 & 713 & 0 & 0.0000 & 274 \\
Phi-4 & PubMedQA & HypMed & 1000 & 321 & 0.3210 & 0 & 0.0000 & 409 & 270 & 993 & 0.9930 & 28 \\
Phi-4 & PubMedQA & Fusion & 1000 & 1 & 0.0010 & 0 & 0.0000 & 290 & 709 & 993 & 0.9930 & 19 \\
\bottomrule
\end{tabular}
